QuadricsReg: Large-Scale Point Cloud Registration using Quadric Primitives

In the realm of large-scale point cloud registration, designing a compact symbolic representation is crucial for efficiently processing vast amounts of data, ensuring registration robustness against significant viewpoint variations and occlusions. This paper introduces a novel point cloud registration method, i.e., QuadricsReg, which leverages concise quadrics primitives to represent scenes and utilizes their geometric characteristics to establish correspondences for 6-DoF transformation estimation. As a symbolic feature, the quadric representation fully captures the primary geometric characteristics of scenes, which can efficiently handle the complexity of large-scale point clouds. The intrinsic characteristics of quadrics, such as types and scales, are employed to initialize correspondences. Then we build a multi-level compatibility graph set to find the correspondences using the maximum clique on the geometric consistency between quadrics. Finally, we estimate the 6-DoF transformation using the quadric correspondences, which is further optimized based on the quadric degeneracy-aware distance in a factor graph, ensuring high registration accuracy and robustness against degenerate structures. We test on 5 public datasets and the self-collected heterogeneous dataset across different LiDAR sensors and robot platforms. The exceptional registration success rates and minimal registration errors demonstrate the effectiveness of QuadricsReg in large-scale point cloud registration scenarios. Furthermore, the real-world registration testing on our self-collected heterogeneous dataset shows the robustness and generalization ability of QuadricsReg on different LiDAR sensors and robot platforms. The codes and demos will be released at \url{https://levenberg.github.io/QuadricsReg}.

==> Contents/Tables/5_4_Evaluation_of_registration_odometry_0.tex <==
% \renewcommand{\arraystretch}{0.8} %
\begin{table*}[t!]
    \label{table: Evaluation of global registration odo}
    \captionsetup{font=footnotesize}
    \centering
    \caption{Evaluation of global registration.(unit: \%).}
    \setlength{\tabcolsep}{4pt}
    {\scriptsize
        \centering
        \begin{tabular}{l|l|ccc|ccc|ccc|ccc|ccc}
            \toprule
            & Dataset & \multicolumn{3}{c|}{KITTI-ODO} & \multicolumn{3}{c|}{KITTI-360-ODO} & \multicolumn{3}{c|}{Apollo-SouthBay-ODO} & \multicolumn{3}{c|}{Waymo-ODO} & \multicolumn{3}{c}{nuScenes-ODO}  \\ \cline{2-17}
            
            & Level & Easy & Medium & Hard & Easy & Medium & Hard & Easy & Medium & Hard & Easy & Medium & Hard & Easy & Medium & Hard \\ \cline{2-17}

            & Pairs & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 & 1000 \\ \cline{1-17}
            
           %  \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{ICP}}}
           % & ICP & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           % & VGICP & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\ \midrule
            
           \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Learning}}}
            & FCGF & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & DGR & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
            & PointDSC & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
            & LCDNet (fast) & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0   \\
            & LCDNet & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\ \cline{1-17}

            \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Point}}} 
           & RANSAC & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & TEASER++ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & Quadro++ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & 3DMAC & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\ \cline{1-17}
           
           \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Geo.}}}
           & Segregator & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & G3Reg & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
           & QuadricsReg & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\ 
           \bottomrule
        \end{tabular}
    }
\end{table*}
